Uncertainty-Resilient Multimodal Learning via Consistency-Guided Cross-Modal Transfer

Multimodal learning systems often face substantial uncertainty due to noisy data, low-quality labels, and heterogeneous modality characteristics. These issues become especially critical in human-computer interaction settings, where data quality, semantic reliability, and annotation consistency vary across users and recording conditions. This thesis tackles these challenges by exploring uncertainty-resilient multimodal learning through consistency-guided cross-modal transfer. The central idea is to use cross-modal semantic consistency as a basis for robust representation learning. By projecting heterogeneous modalities into a shared latent space, the proposed framework mitigates modality gaps and uncovers structural relations that support uncertainty estimation and stable feature learning. Building on this foundation, the thesis investigates strategies to enhance semantic robustness, improve data efficiency, and reduce the impact of noise and imperfect supervision without relying on large, high-quality annotations. Experiments on multimodal affect-recognition benchmarks demonstrate that consistency-guided cross-modal transfer significantly improves model stability, discriminative ability, and robustness to noisy or incomplete supervision. Latent space analyses further show that the framework captures reliable cross-modal structure even under challenging conditions. Overall, this thesis offers a unified perspective on resilient multimodal learning by integrating uncertainty modeling, semantic alignment, and data-efficient supervision, providing practical insights for developing reliable and adaptive brain-computer interface systems.

==> appendices.tex <==
% \input{chapters/appendix_codes}

==> beginnings/acknowledgement.tex <==
This research was supported by the Institute of Information \& Communications Technology Planning \& Evaluation (IITP) grant, funded by the Korea government (MSIT) (No. RS-2019-II190079 (Artificial Intelligence Graduate School Program (Korea University)), and No. RS-2024-00457882 (AI Research Hub Project)).

==> beginnings/enabstract.tex <==
\input{MAIN_Variables}

Multimodal learning systems must operate under significant uncertainty arising from noisy data, low-quality labels, and heterogeneous modality characteristics. These challenges become particularly critical in human–computer interaction contexts, where data quality, semantic reliability, and annotation consistency often fluctuate across user-driven variations and recording conditions. This thesis addresses these limitations by exploring uncertainty-resilient multimodal learning through consistency-guided cross-modal transfer, aiming to develop models that remain stable and reliable under imperfect supervision.
The core idea of this work is to leverage cross-modal semantic consistency as a foundation for robust representation learning. By projecting heterogeneous modalities into a shared latent space, the proposed framework mitigates modality gaps and reveals structural relationships that support both uncertainty estimation and stable feature learning. Building on this foundation, the thesis investigates strategies that enhance semantic robustness, improve data efficiency, and reduce the impact of noise and label imperfections—without relying on large-scale, high-quality annotations.
Empirical evaluations on multimodal affect recognition benchmarks demonstrate that consistency-guided cross-modal transfer substantially improves model stability, discriminative power, and robustness to noisy or incomplete supervision. Latent-space analyses further show that the framework effectively captures reliable cross-modal structure even under challenging data conditions.
Overall, this thesis provides a unified perspective on resilient multimodal learning by integrating uncertainty modeling, semantic alignment, and data-efficient supervision. The findings offer practical insights and scalable methodologies for developing robust multimodal systems that support more reliable and adaptive brain-computer interfaces.


% \vspace*{\fill}
{\bf Keywords:} Brain-computer interfaces, Multimodal learning, Active learning, Knowledge distillation, Uncertainty

==> beginnings/krabstract.tex <==
다중모달 학습 시스템은 잡음이 포함된 데이터, 저품질의 레이블, 그리고 이질적인 모달리티 특성으로부터 발생하는 다양한 불확실성 속에서 동작해야 한다. 이러한 문제는 인간–컴퓨터 상호작용 환경에서 특히 두드러지는데, 데이터 품질, 의미적 신뢰성, 그리고 레이블 일관성이 사용자 요인에 따른 변동성과 기록 조건의 차이에 따라 쉽게 흔들리기 때문이다. 본 논문은 이러한 한계를 해결하기 위해 모달리티 간 일관성에 기반한 교차모달 전이를 활용한 불확실성에 대응하는 다중모달 학습을 탐구하며, 불완전한 감독 환경에서도 안정적이고 신뢰할 수 있는 모델을 구축하는 것을 목표로 한다.
본 연구의 핵심은 상이한 모달리티 간의 의미적 일관성을 활용하여 강건한 표현을 학습하는 것이다. 다양한 모달리티를 공유 잠재 공간으로 투영함으로써 모달리티 간 격차를 완화하고, 불확실성 추정 및 안정적 특징 학습을 가능하게 하는 구조적 패턴을 추출한다. 이러한 기반 위에서 본 논문은 대규모 고품질 레이블에 의존하지 않으면서도 의미적 안정성 향상, 데이터 효율성 개선, 레이블 오류 감소를 달성할 수 있는 전략을 제안한다.
다중모달 감정 인식 벤치마크를 활용한 실험 결과, 제안한 접근법은 기존의 단일모달 및 다중모달 기법에 비해 모델의 안정성, 판별력, 그리고 노이즈나 불완전한 감독에 대한 강건성을 크게 향상시킴을 확인하였다. 또한, 잠재 표현 분석을 통해, 제안된 프레임워크가 다양한 데이터 조건에서도 신뢰할 수 있는 모달리티 간 구조를 효과적으로 학습함을 추가적으로 검증하였다.
종합적으로, 본 논문은 불확실성 추정, 의미 정합, 데이터 효율적 감독을 통합한 강건한 다중모달 학습 전략을 제안한다. 이러한 연구 결과는 실제 환경에서 더욱 안정적이고 적응적인 뇌–컴퓨터 인터페이스 시스템 개발을 위한 실질적인 통찰과 확장 가능한 방법론을 제시한다.

% \vspace*{\fill}
{\bf 주제어:} 뇌-컴퓨터 인터페이스, 다중모달 학습, 능동 학습, 지식 증류, 불확실성

==> beginnings/preface.tex <==
This dissertation is submitted for the degree of Master of Science in Brain and Cognitive Engineering at Korea University.
The research described herein was conducted under the supervision of Professor Seong-Whan Lee in the Department of Artificial Intelligence, Korea University. Part of this thesis was submitted as a conference paper and presented at the IEEE International Conference on Systems, Man, and Cybernetics (SMC) 2025. I was the lead investigator for the projects where I was responsible for all major areas of concept formation, data collection and analysis, as well as the majority of manuscript composition. Neither this, nor any substantially similar dissertation has been or is being submitted for any other degree, diploma, or other qualification at any other university.

==> chapters/MAIN_Variables.tex <==
% \renewcommand{\methodname}{STAARS}
% \renewcommand{\weightcomponent}{class-specific multiplier}
